Enhanced Meta Reinforcement Learning using Demonstrations in Sparse Reward Environments

Meta reinforcement learning (Meta-RL) is an approach wherein the experience gained from solving a variety of tasks is distilled into a meta-policy. The meta-policy, when adapted over only a small (or just a single) number of steps, is able to perform near-optimally on a new, related task. However, a major challenge to adopting this approach to solve real-world problems is that they are often associated with sparse reward functions that only indicate whether a task is completed partially or fully. We consider the situation where some data, possibly generated by a sub-optimal agent, is available for each task. We then develop a class of algorithms entitled Enhanced Meta-RL using Demonstrations (EMRLD) that exploit this information even if sub-optimal to obtain guidance during training. We show how EMRLD jointly utilizes RL and supervised learning over the offline data to generate a meta-policy that demonstrates monotone performance improvements. We also develop a warm started variant called EMRLD-WS that is particularly efficient for sub-optimal demonstration data. Finally, we show that our EMRLD algorithms significantly outperform existing approaches in a variety of sparse reward environments, including that of a mobile robot.

==> sections/experiments_1.tex <==
\section{Experimental Evaluation}
In this section we evaluate the performance of our algorithm and aim to answer the following questions: 1) Can demonstration data help in learning meta policies in sparse reward environments? 2) Do the demonstrations have to be optimal? 3) How well does the meta policy adapt to unseen tasks? We exhaustively analyse the performance of our algorithm on \textit{sparse} multi-task versions of simulated continuous control environments with tasks that differ in their reward functions. These environments include,  Point2D Navigation \cite{finn2017model}, TwoWheeled Locomotion \cite{gupta2018meta}, and HalfCheetah \cite{wawrzynski2009cat, todorov2012mujoco}.  We further demonstrate the superior performance of our algorithm in a sparse reward environment where the tasks differ in their dynamics. We then evaluate our algorithm in the real world, using a TurtleBot (A two-wheeled differential drive robot)\cite{amsters2019turtlebot} and demonstrate that it can adapt to a new unseen task by collecting a few trajectories and just one step of adaptation.
% \begin{enumerate}
%     \item When MAML fails in sparse environments, can offline data assist learning of desirable meta policies?
%     \item Does the data have to come from an optimal expert? Can learning take place with highly sub-optimal data? 
%     \item Does data help in environments that are not goal reaching?
%     \item Does assistance of data become apparent in real robotic tasks? 
%     \item Does our learned meta policy generalize to unseen tasks? 
%     %\item Do we observe monotone improvement in practise? 
%     %\item \textcolor{red}{Performance with amount of data - does having more data help?}
%     %\item \textcolor{red}{Does structure in expert data help in any way?}
%     %\item \textcolor{red}{What happens the sparsity is different for different tasks?}
% \end{enumerate}
 
\subsection{Experiments on simulated domains}
\begin{wrapfigure}{r}{0.22\textwidth}
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[width=\linewidth,trim=20 0 120 5,clip]{NeurIPS_2022/sections/figures/simulated_envs/point_env.pdf}
\vskip
\includegraphics[width=\linewidth, trim=20 0 120 5,clip]{NeurIPS_2022/sections/figures/simulated_envs/wheeled_env.pdf}
\vskip
\includegraphics[width=\linewidth, trim=10 0 10 100,clip]{NeurIPS_2022/sections/figures/simulated_envs/hc_gym.jpeg}
\end{subfigure}
\vskip\baselineskip
\caption{Simulated environments.}
\end{wrapfigure}
\paragraph{Sparse multi-task environments} We train on standard meta-reinforcement learning environments Point2D Navigation, TwoWheeled Locomotion, and Half Cheetah Forward-Backward\cite{finn2017model, gupta2018meta, wawrzynski2009cat, todorov2012mujoco} with modified reward functions or dynamics. We work with multi-task versions of these environments where we fix the number of tasks to a finite small number, and repeatedly train on these fixed tasks. This is reasonable since in practice we do not encounter thousands of similar tasks to meta-train on, and collecting demonstration data for a large number of task is impractical. 

\textit{Point2D Navigation} is a 2 dimensional goal reaching environment. The states are $(x,y)$ location of the agent on a 2D plane. The actions are appropriate 2D displacements $(dx,dy)$. Tasks are defined by a fixed set of $12$ goal locations on a semi-circle of radius $2$. The agent is given a zero reward everywhere except when it is a certain distance near the goal location, making the reward function highly \textit{sparse}. Within a single task, the objective of the agent is to reach the goal location in the least number of time steps starting from origin. A good meta-policy is expected to adapt and perform well on any of these $12$ goals, and possibly on out-of-sample goals. The \textit{TwoWheeled Locomotion} environment is a goal-reaching with sparse reward, similar to Point2D Navigation. Here, we work with a fixed set of $24$ goal locations on a semi-circle of radius $2$. Further details on state-space and dynamics are provided in the Appendix. \textit{HalfCheetah Forward-Backward} consists two tasks: HalfCheetah agent learning to move in the forward (task 1) and the backward (task 2) directions with as high velocity as possible. The agent gets reward only after it has moved a certain number of units along the x-axis in the correct direction, making the rewards sparse. 

%The agent gets a sparse reward feedback: no reward till the agent moves a certain number of units along the x-axis. 


\paragraph{Optimal data and sub-optimal data} \begin{wrapfigure}{r}{0.5\textwidth}
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[width=0.45\linewidth]{NeurIPS_2022/sections/figures/explanation/Good.pdf}
\includegraphics[width=0.45\linewidth]{NeurIPS_2022/sections/figures/explanation/Bad.pdf}
\end{subfigure}
\vskip\baselineskip
\caption{Optimal  data and Sub-optimal data.}
\end{wrapfigure} We overcome the impairment induced by sparse rewards in meta-reinforcement learning by using limited amount of available demonstration data: just one trajectory per task for guidance. We work with two kinds of demonstration data - optimal and sub-optimal data. Optimal data consists of  $(s,a)$ transitions sampled from an optimal expert policy trained using TRPO. Sub-optimal demonstration data consists of $(s,a)$ transitions sampled from a partially trained  TRPO policy with induced action noises and truncated trajectories. 

\paragraph{Training and testing} During meta training, the algorithm is only exposed to the training tasks ($12$ for Point2D Navigation, $24$ for TwoWheeled Locomotion, and two for HalfCheetah Forward-Backward) and the data associated with these tasks. During testing, we sample tasks at random from the task distribution from which the original training tasks were sampled, and collect the same amount of demonstration data as done during the training phase. For the \textit{Point2D Navigation}  and \textit{TwoWheeled Locomotion} environments, we sample $20$ random goal points on the semi-circle of radius $2$. For the  \textit{HalfCheetah Forward-Backward}, the testing tasks are the same as the training tasks.

\textbf{Baselines}  We compare the performance of our algorithm against the following gradient based meta-reinforcement learning algorithms: (i) \textbf{MAML:} \cite{finn2017model} The standard MAML algorithm for meta-reinforcement learning (ii) \textbf{Meta-BC:} \cite{finn2017one} Supervised learning/Behavior cloning version of MAML, where the maximum likelihood loss is used in the adaptation as well as the meta-update steps. (iii) \textbf{GMPS:} \cite{mendonca2019guided} Guided meta policy search, a gradient based meta reinforcement learning algorithm that uses demonstration data only for its meta parameter update. 

\subsubsection{Performance with optimal data}
We report the training and testing/generalization performance of our algorithms and baselines trained and tested with optimal data in figure \ref{fig:good_data_train_adapt}. In the top row of figure \ref{fig:good_data_train_adapt}, we plot the average adapted return across training tasks of the meta-policy during training iterations. In the bottom row of figure \ref{fig:good_data_train_adapt}, we plot the average adapted return of the trained meta policy adapted across testing tasks over adaptation steps. Note that in all the three environments, our algorithms out preform the other baselines by obtaining the highest average return, and are able to quickly adapt to testing tasks with just one adaptation step and one trajectory of demonstration data. Additionally, our algorithms demonstrate nearly-monotone improvement in average return demonstrating stable learning. Meta-BC fails and has unstable training performance as the amount of demonstration data available per task is very small. The presence of fewer training task further hampers the  performance of Meta-BC. MAML and GMPS fail to learn due to sparsity of the environment as the purely RL adaptation step incurs almost zero reward, and hence, negligible learning signal.

In Fig. \ref{fig:good_data_train_adapt}b, we include the testing performance. 

\subsubsection{Performance on bad data}
We wish to demonstrate the benefit the of the RL component of our algorithm which is present in both the adaptation as well as meta update steps. To do so,  we evaluate the performance of our algorithm when exposed to sub-optimal demonstration data. For the  Point2D Navigation environment, we collect one trajectory per task (12 in total) using a partially trained agent, with induced action noise. We further truncate the trajectories outside the reward region to ensure that simply mimicking the data, will not reach the goal. For the TwoWheeled Locomotion environment, we collect data in a similar fashion for all the 24 tasks, but remove state-action pairs at the beginning of each trajectory. We do so, since the first few state action pairs contains information on how to orient the two-wheeled agent towards the goal, and this information is crucial for reaching the goal. We note that our algorithm outperforms all the baselines, emphasizing the benefit of the RL component in our algorithm.   BC-Avg, GMPS, and WTL fail because they are restricted by the optimality of the data, and the absence of crucial information greatly impacts their performance. MAML fails due to the sparsity of the reward.  

\input{NeurIPS_2022/sections/figures_tex/traj_plot}
\input{NeurIPS_2022/sections/figures_tex/good_data_train_adapt}
\input{NeurIPS_2022/sections/figures_tex/bad_data_train_adapt}

\subsection{Experiments on TurtleBot}
For the changing dynamics setting, we modify the \textit{TwoWheeled Locomotion} sparse reward environment wherein we fix the goal, but change the dynamics by inducing  angular velocity which mimics drifts in the environment. We train on a fixed set of $9$ different angular velocity values, further details are included in the Appendix.      

\input{NeurIPS_2022/sections/figures_tex/turtlebot_figure}


==> sections/figures_tex/bad_data_training.tex <==
\begin{figure*}[h]
\centering
\includegraphics[width=0.32\linewidth]{NeurIPS_2022/sections/figures/bad_data/Point2D_bad.pdf}
\hfill
\includegraphics[width=0.32\linewidth]{NeurIPS_2022/sections/figures/bad_data/2Wheeled_bad.pdf}
\hfill
\includegraphics[width=0.32\linewidth]{NeurIPS_2022/sections/figures/bad_data/HC_bad.pdf} %, trim = 50 10 100 100, clip
\caption{Experiments on 2D Navigation, Wheeled locomotion and Half Cheetah when the demonstration data is from a bad expert}
% \label{fig:MuJoCo_Full_Ob}
\end{figure*}

==> sections/figures_tex/good_data_training.tex <==
\begin{figure*}[h]
\centering
\begin{subfigure}{\linewidth}
    \centering
    \includegraphics[width=0.85\linewidth,trim=110 10 90 10,clip]{NeurIPS_2022/sections/figures/legend/legend.pdf}
\end{subfigure}
\vskip\baselineskip
\begin{subfigure}{\linewidth}
\centering
\includegraphics[width=0.32\linewidth]{NeurIPS_2022/sections/figures/good_data/Point2D_good.pdf}
\hfill
\includegraphics[width=0.32\linewidth]{NeurIPS_2022/sections/figures/good_data/2Wheeled_good.pdf}
\hfill
\includegraphics[width=0.32\linewidth,trim=0 0 0 5,clip]{NeurIPS_2022/sections/figures/good_data/HC_good.pdf} %trim = 50 10 100 100, clip
\caption{Good data}
\end{subfigure}
\vskip\baselineskip

\begin{subfigure}{\linewidth}
\centering
\includegraphics[width=0.32\linewidth]{NeurIPS_2022/sections/figures/bad_data/Point2D_bad.pdf}
\hfill
\includegraphics[width=0.32\linewidth]{NeurIPS_2022/sections/figures/bad_data/2Wheeled_bad.pdf}
\hfill
\includegraphics[width=0.32\linewidth]{NeurIPS_2022/sections/figures/bad_data/HC_bad.pdf} %, trim = 50 10 100 100, clip
\caption{Bad data}
\end{subfigure}
\caption{Experiments on 2D Navigation, Wheeled locomotion and Half Cheetah when the demonstration data is (a) from a good expert, and (b) from a bad expert. All the plots are averaged over three random seeds.}
\label{fig:training_curves}
\end{figure*}



==> sections/figures_tex/particle.tex <==

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{icml2022/figures/point2d/expert_demos.png}
%     \caption{Expert demo data. (a) Bad demonstration data (b) Good demo data}
%     \label{fig:my_label}
% \end{figure}
% \begin{figure*}[b!]
% \centering
% \begin{subfigure}{\linewidth}
% \centering
% \includegraphics[width=0.19\linewidth]{icml2022/figures/point2d/Very_Good_12.pdf}
% \hfill
% \includegraphics[width=0.19\linewidth]{icml2022/figures/point2d/BC_A2C_TRPO_Policy_Very_Good_12_data_Very_Good_12_adapt_steps_2.pdf}
% \hfill
% \includegraphics[width=0.19\linewidth]{icml2022/figures/point2d/BC_TRPO_Policy_Very_Good_12_data_Very_Good_12_adapt_steps_2.pdf}
% \hfill
% \includegraphics[width=0.19\linewidth]{icml2022/figures/point2d/BC_AVG_Policy_Very_Good_12_data_Very_Good_12_adapt_steps_1.pdf}
% \hfill
% \includegraphics[width=0.19\linewidth]{icml2022/figures/point2d/MAML_Policy_Very_Good_12_data_Very_Good_12_adapt_steps_1.pdf}
% \caption{Good 12 point data}
% % \label{fig:MuJoCo_Full_Ob}
% \end{subfigure}
% \vskip\baselineskip
% \begin{subfigure}{\linewidth}
% \centering
% \includegraphics[width=0.19\linewidth]{icml2022/figures/point2d/Very_Good_random_3_100.pdf}
% \hfill
% \includegraphics[width=0.19\linewidth]{icml2022/figures/point2d/BC_A2C_TRPO_Policy_Very_Good_12_data_Very_Good_random_3_100_adapt_steps_2.pdf}
% \hfill
% \includegraphics[width=0.19\linewidth]{icml2022/figures/point2d/BC_TRPO_Policy_Very_Good_12_data_Very_Good_random_3_100_adapt_steps_2.pdf}
% \hfill
% \includegraphics[width=0.19\linewidth]{icml2022/figures/point2d/BC_AVG_Policy_Very_Good_12_data_Very_Good_random_3_100_adapt_steps_1.pdf}
% \hfill
% \includegraphics[width=0.19\linewidth]{icml2022/figures/point2d/MAML_Policy_Very_Good_12_data_Very_Good_random_3_100_adapt_steps_1.pdf}
% \caption{Good 100 data}
% % \label{fig:MuJoCo_Inc_Ob}
% \end{subfigure}
% \vskip\baselineskip
% \begin{subfigure}{\linewidth}
% \centering
% \includegraphics[width=0.19\linewidth]{icml2022/figures/point2d/Bad_random_3_100.pdf}
% \hfill
% \includegraphics[width=0.19\linewidth]{icml2022/figures/point2d/BC_A2C_TRPO_Policy_Very_Good_12_data_Bad_random_3_100_adapt_steps_4.pdf}
% \hfill
% \includegraphics[width=0.19\linewidth]{icml2022/figures/point2d/BC_TRPO_Policy_Very_Good_12_data_Bad_random_3_100_adapt_steps_4.pdf}
% \hfill
% \includegraphics[width=0.19\linewidth]{icml2022/figures/point2d/BC_AVG_Policy_Very_Good_12_data_Bad_random_3_100_adapt_steps_2.pdf}
% \hfill
% \includegraphics[width=0.19\linewidth]{icml2022/figures/point2d/MAML_Policy_Very_Good_12_data_Bad_random_3_100_adapt_steps_2.pdf}
% \caption{Bad 100 data}
% % \label{fig:MuJoCo_Inc_Ob}
% \end{subfigure}


% \caption{Test}
% \end{figure*}



\begin{figure*}[b!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[width=0.3\linewidth]{NeurIPS_2022/sections/figures/point_adaptation/good_data/Very_Good_12.pdf}
\hfill
\includegraphics[width=0.3\linewidth]{NeurIPS_2022/sections/figures/point_adaptation/good_data/Very_Good_random_50.pdf}
\hfill
\includegraphics[width=0.3\linewidth]{NeurIPS_2022/sections/figures/point_adaptation/good_data/Good_Data_Adapt.pdf}
\caption{Good 12 point}
\end{subfigure}
\vskip\baselineskip

\begin{subfigure}{\linewidth}
\centering
\includegraphics[width=0.3\linewidth]{NeurIPS_2022/sections/figures/point_adaptation/MAML_Policy_data_Very_Good_random_50_adapt_steps_0.pdf}
\hfill
\includegraphics[width=0.3\linewidth]{NeurIPS_2022/sections/figures/point_adaptation/MAML_Policy_data_Very_Good_random_50_adapt_steps_1.pdf}
\hfill
\includegraphics[width=0.3\linewidth]{NeurIPS_2022/sections/figures/point_adaptation/MAML_Policy_data_Very_Good_random_50_adapt_steps_3.pdf}
\caption{MAML adapted on 50 random points}
\end{subfigure}

\vskip\baselineskip

\begin{subfigure}{\linewidth}
\centering
\includegraphics[width=0.3\linewidth]{NeurIPS_2022/sections/figures/point_adaptation/good_data/BC_TRPO_Policy_data_Very_Good_random_50_adapt_steps_0.pdf}
\hfill
\includegraphics[width=0.3\linewidth]{NeurIPS_2022/sections/figures/point_adaptation/good_data/BC_TRPO_Policy_data_Very_Good_random_50_adapt_steps_1.pdf}
\hfill
\includegraphics[width=0.3\linewidth]{NeurIPS_2022/sections/figures/point_adaptation/good_data/BC_TRPO_Policy_data_Very_Good_random_50_adapt_steps_3.pdf}
\caption{BC TRPO adapted on 50 random points with good data}
\end{subfigure}

\begin{subfigure}{\linewidth}
\centering
\includegraphics[width=0.3\linewidth]{NeurIPS_2022/sections/figures/point_adaptation/good_data/BC_A2C_TRPO_Policy_data_Very_Good_random_50_adapt_steps_0.pdf}
\hfill
\includegraphics[width=0.3\linewidth]{NeurIPS_2022/sections/figures/point_adaptation/good_data/BC_A2C_TRPO_Policy_data_Very_Good_random_50_adapt_steps_1.pdf}
\hfill
\includegraphics[width=0.3\linewidth]{NeurIPS_2022/sections/figures/point_adaptation/good_data/BC_A2C_TRPO_Policy_data_Very_Good_random_50_adapt_steps_3.pdf}
\caption{BC+A2C TRPO adapted on 50 random points with good data}
\end{subfigure}
\caption{Good Data point2d}
\end{figure*}

\begin{figure*}[b!]
\centering
\vskip\baselineskip
\begin{subfigure}{\linewidth}
\centering
\includegraphics[width=0.3\linewidth]{NeurIPS_2022/sections/figures/point_adaptation/bad_data/Bad_12.pdf}
\hfill
\includegraphics[width=0.3\linewidth]{NeurIPS_2022/sections/figures/point_adaptation/bad_data/Bad_random_50.pdf}
\hfill
\includegraphics[width=0.3\linewidth]{NeurIPS_2022/sections/figures/point_adaptation/bad_data/Bad_Data_Adapt.pdf}
\caption{Bad 12 point}
\end{subfigure}

\begin{subfigure}{\linewidth}
\centering
\includegraphics[width=0.3\linewidth]{NeurIPS_2022/sections/figures/point_adaptation/bad_data/BC_TRPO_Policy_data_Bad_random_50_adapt_steps_0.pdf}
\hfill
\includegraphics[width=0.3\linewidth]{NeurIPS_2022/sections/figures/point_adaptation/bad_data/BC_TRPO_Policy_data_Bad_random_50_adapt_steps_1.pdf}
\hfill
\includegraphics[width=0.3\linewidth]{NeurIPS_2022/sections/figures/point_adaptation/bad_data/BC_TRPO_Policy_data_Bad_random_50_adapt_steps_3.pdf}
\caption{BC TRPO adapted on 50 random points with bad data}
\end{subfigure}

\begin{subfigure}{\linewidth}
\centering
\includegraphics[width=0.3\linewidth]{NeurIPS_2022/sections/figures/point_adaptation/bad_data/BC_A2C_TRPO_Policy_data_Bad_random_50_adapt_steps_0.pdf}
\hfill
\includegraphics[width=0.3\linewidth]{NeurIPS_2022/sections/figures/point_adaptation/bad_data/BC_A2C_TRPO_Policy_data_Bad_random_50_adapt_steps_1.pdf}
\hfill
\includegraphics[width=0.3\linewidth]{NeurIPS_2022/sections/figures/point_adaptation/bad_data/BC_A2C_TRPO_Policy_data_Bad_random_50_adapt_steps_3.pdf}
\caption{BC-A2C TRPO adapted on 50 random points with bad data}
\end{subfigure}

\caption{Point2d with bad data}
\end{figure*}

==> sections/figures_tex/simulated_envs.tex <==
\begin{figure*}[!h]
\begin{subfigure}{\linewidth}
\centering
\includegraphics[width=0.27\linewidth]{NeurIPS_2022/sections/figures/turtle_bot/turtle_bot_hw.png}
\hfill
\includegraphics[width=0.37\linewidth]{NeurIPS_2022/sections/figures/turtle_bot/turtlebot_500.pdf}
\hfill
\includegraphics[width=0.30\linewidth,trim=0 0 0 5,clip]{NeurIPS_2022/sections/figures/turtle_bot/Turtlebot_testing.pdf}
\end{subfigure}
\caption{Turtlebot results}
\label{fig:good_data_train_adapt}
\end{figure*}

==> sections/figures_tex/two_wheeled.tex <==
\begin{figure*}[b!]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[width=0.3\linewidth]{NeurIPS_2022/sections/figures/two_wheeled_adaptation/good_data/Very_Good_24.pdf}
\hfill
\includegraphics[width=0.3\linewidth]{NeurIPS_2022/sections/figures/two_wheeled_adaptation/good_data/Very_Good_random_50.pdf}
\hfill
\includegraphics[width=0.3\linewidth]{NeurIPS_2022/sections/figures/two_wheeled_adaptation/good_data/Good_Data_Adapt_TwoWheel.pdf}
\caption{Good 24 point}
\end{subfigure}
\vskip\baselineskip

\begin{subfigure}{\linewidth}
\centering
\includegraphics[width=0.3\linewidth]{NeurIPS_2022/sections/figures/two_wheeled_adaptation/MAML_Policy_data_Very_Good_random_50_adapt_steps_0.pdf}
\hfill
\includegraphics[width=0.3\linewidth]{NeurIPS_2022/sections/figures/two_wheeled_adaptation/MAML_Policy_data_Very_Good_random_50_adapt_steps_1.pdf}
\hfill
\includegraphics[width=0.3\linewidth]{NeurIPS_2022/sections/figures/two_wheeled_adaptation/MAML_Policy_data_Very_Good_random_50_adapt_steps_3.pdf}
\caption{MAML adapted on 50 random points}
\end{subfigure}

\vskip\baselineskip

\begin{subfigure}{\linewidth}
\centering
\includegraphics[width=0.3\linewidth]{NeurIPS_2022/sections/figures/two_wheeled_adaptation/good_data/BC_TRPO_Policy_data_Very_Good_random_50_adapt_steps_0.pdf}
\hfill
\includegraphics[width=0.3\linewidth]{NeurIPS_2022/sections/figures/two_wheeled_adaptation/good_data/BC_TRPO_Policy_data_Very_Good_random_50_adapt_steps_1.pdf}
\hfill
\includegraphics[width=0.3\linewidth]{NeurIPS_2022/sections/figures/two_wheeled_adaptation/good_data/BC_TRPO_Policy_data_Very_Good_random_50_adapt_steps_3.pdf}
\caption{BC TRPO adapted on 50 random points with good data}
\end{subfigure}

\begin{subfigure}{\linewidth}
\centering
\includegraphics[width=0.3\linewidth]{NeurIPS_2022/sections/figures/two_wheeled_adaptation/good_data/BC_A2C_TRPO_Policy_data_Very_Good_random_50_adapt_steps_0.pdf}
\hfill
\includegraphics[width=0.3\linewidth]{NeurIPS_2022/sections/figures/two_wheeled_adaptation/good_data/BC_A2C_TRPO_Policy_data_Very_Good_random_50_adapt_steps_1.pdf}
\hfill
\includegraphics[width=0.3\linewidth]{NeurIPS_2022/sections/figures/two_wheeled_adaptation/good_data/BC_A2C_TRPO_Policy_data_Very_Good_random_50_adapt_steps_3.pdf}
\caption{BC+A2C TRPO adapted on 50 random points with good data}
\end{subfigure}
\caption{Good Data Two Wheeled}
\end{figure*}

\begin{figure*}[b!]
\centering
\vskip\baselineskip
\begin{subfigure}{\linewidth}
\centering
\includegraphics[width=0.3\linewidth]{NeurIPS_2022/sections/figures/two_wheeled_adaptation/bad_data/Bad_24.pdf}
\hfill
\includegraphics[width=0.3\linewidth]{NeurIPS_2022/sections/figures/two_wheeled_adaptation/bad_data/Bad_random_50.pdf}
\hfill
\includegraphics[width=0.3\linewidth]{NeurIPS_2022/sections/figures/two_wheeled_adaptation/bad_data/Bad_Data_Adapt_TwoWheel.pdf}
\caption{Bad 24 point}
\end{subfigure}

\begin{subfigure}{\linewidth}
\centering
\includegraphics[width=0.3\linewidth]{NeurIPS_2022/sections/figures/two_wheeled_adaptation/bad_data/BC_TRPO_Policy_data_Bad_random_50_adapt_steps_0.pdf}
\hfill
\includegraphics[width=0.3\linewidth]{NeurIPS_2022/sections/figures/two_wheeled_adaptation/bad_data/BC_TRPO_Policy_data_Bad_random_50_adapt_steps_1.pdf}
\hfill
\includegraphics[width=0.3\linewidth]{NeurIPS_2022/sections/figures/two_wheeled_adaptation/bad_data/BC_TRPO_Policy_data_Bad_random_50_adapt_steps_3.pdf}
\caption{BC TRPO adapted on 50 random points with bad data}
\end{subfigure}

\begin{subfigure}{\linewidth}
\centering
\includegraphics[width=0.3\linewidth]{NeurIPS_2022/sections/figures/two_wheeled_adaptation/bad_data/BC_A2C_TRPO_Policy_data_Bad_random_50_adapt_steps_0.pdf}
\hfill
\includegraphics[width=0.3\linewidth]{NeurIPS_2022/sections/figures/two_wheeled_adaptation/bad_data/BC_A2C_TRPO_Policy_data_Bad_random_50_adapt_steps_1.pdf}
\hfill
\includegraphics[width=0.3\linewidth]{NeurIPS_2022/sections/figures/two_wheeled_adaptation/bad_data/BC_A2C_TRPO_Policy_data_Bad_random_50_adapt_steps_3.pdf}
\caption{BC-A2C TRPO adapted on 50 random points with bad data}
\end{subfigure}

\caption{Two Wheeled with bad data}
\end{figure*}



==> sections/introduction_1.tex <==
\section{Introduction}
\sap{None of the figures are final. Please suggest changes and corrections.} 
Points to cover
\begin{enumerate}
    \item What are mult-task problems in reinforcement learning? Why are such problems important to solve? (Look at distillation and multi-task papers)
    \item What is model agnostic meta learning, why is it the go-to algorithm for multi-tasking? 
    \item Why MAML would fail in sparse environments? 
    \item Data has been used in the past to get RL algorithms to work better in sparsely rewarded environments. 
    \item We propose to use data in MAML
    \item How are we different from WTL
    \item List shortcomings of HTR - it is goal based. 
\end{enumerate}

Deep reinforcement learning (Deep RL or DRL) algorithms are data inefficient in complex high dimensional environments. To overcome data in-efficency, multi-task reinforcement learning has been studied with the hope of learning from the shared knowledge across tasks. Here, the shared knowledge typically comes in the form of reward function or environment dynamics. In this work, our focus is on RL tasks that share the same environment dynamics. 

Model agnostic meta learning for reinforcement learning (MAML-RL) \cite{finn2017model} was proposed as a learning-to-learn based solution for multi-task RL, and has since become the go-to algorithm for multi-task RL problems. MAML-RL is a gradient based on-policy algorithm that aims to learn a meta-policy that can quickly adapt to a task-specific policy using minimal task specific data. The meta-policy interacts with the task specific environments to obtain task specific data, and then updates meta-policy parameters using this task specific data and a suitable loss function. So, essentially the learning signal comes from the collected task specific data. In rich densely rewarded environments, this task specific data is per time step reward. Thus, gradient based MAML-RL heavily relies on richness of the reward function. However, sparsely rewarded environments are more prevalent in the wild. In sparsely rewarded environments, the agent receives the reward signal at only few time steps over the course of agent run. MAML, by the nature of construction of algorithm (as explained above), would fail in sparsely rewarded environments due to the lack of rich learning signal in terms of every time-step reward. 

To deal with the sparse rewards setting in RL, learning from demonstrations (LfD) was proposed. LfD deals with sparsity by including minimal expert demonstration data during the course of RL agent training. List and describe all the LfD methods in short. 

Taking inspiration from the success of LfD in single task RL, in this work we propose two algorithms - MLfD-0 and MLfD-1 - to obtain a meta-policy for tasks with sparse rewards.  

==> sections/tables/avg_1_step_adaptation.tex <==

    \begin{table*}[t]
    %   \vspace{-1.5\baselineskip}
    %   \newcolumntype{g}{>{\columncolor{gray!15}}c}
      \caption{Average 1-step adaptation reward of policies trained using bad demo data. Both training and testing are done on sparse environments. MAML-RL \cite{finn2017model}, WTL \cite{zhou2019watch}}
      \label{bench-results-table}
      \centering
      \setlength\tabcolsep{3.3pt}
      \begin{tabular}{c|c|c|| c|c|| c|c}
        \hline
          & \multicolumn{6}{c}{Environment} \\ \cline{2-7} 
        Algorithm   &  \multicolumn{2}{c||}{Point 2D}     &      \multicolumn{2}{c||}{Wheeled Locomotion}   & \multicolumn{2}{c}{Ant-v3}  \\ \cline{2-7}
          & 12 Goals & 24 Goals & 12 Goals & 24 Goals & 12 Goals & 24 Goals \\ \hline
        % \multicolumn{9}{c}{Vanilla Algorithms} \\ \hline
        MAML-RL & $ -145.56 \pm 10.64$ & $47.6 \pm 10.64$   & $ 217.04 \pm 51.61$ & $34.9 \pm 1.36$     & $ -4.26 \pm 0.25 $ & $4.56 \pm 0.45$  \\ \hline 
        MLfD-0 (Ours)   & $ -139.86 \pm 8.29$  & $9.32 \pm 1.13$    & $277.62 \pm 11.02$     & $8.14 \pm 0.81$     & $-5.96 \pm 0.47$   & $5.99 \pm 0.91$ \\ \hline 
        MLfD-1 (Ours)  & $-152.71 \pm 9.47$   & $43.9 \pm 30.94$   & $271.06 \pm 17.39$  & $37.9 \pm 12.30$    & $-6.52 \pm 1.12$      & $5.70 \pm 0.98$ \\ \hline 
        BC-Average   & $-668.60 \pm 551.85 $   & $9.29 \pm 5.51$    & $ 169.08 \pm 56.59$ & $11.4 \pm 1.36$     & $ -4.37 \pm 1.74$  & $4.49 \pm 0.43$    \\ \hline 
        WTL & \cellcolor{green!11} $-590.35 \pm 295.86$ & \cellcolor{green!12} $8.09 \pm 2.13$ & \cellcolor{red!17} $140.71 \pm 23.03 $    & \cellcolor{green!12} $10.0 \pm 2.92$  & \cellcolor{red!8} $-4.69 \pm 2.05$      & \cellcolor{green!24} $ 3.38 \pm 0.36$ \\ \hline
        \end{tabular}
        \vspace{-1.8\baselineskip}
    \end{table*}
    
